Semixup: In- and Out-of-Manifold Regularization for Deep Semi-Supervised Knee Osteoarthritis Severity Grading from Plain Radiographs

Knee osteoarthritis (OA) is one of the highest disability factors in the world. This musculoskeletal disorder is assessed from clinical symptoms, and typically confirmed via radiographic assessment. This visual assessment done by a radiologist requires experience, and suffers from moderate to high inter-observer variability. The recent literature has shown that deep learning methods can reliably perform the OA severity assessment according to the gold standard Kellgren-Lawrence (KL) grading system. However, these methods require large amounts of labeled data, which are costly to obtain. In this study, we propose the Semixup algorithm, a semi-supervised learning (SSL) approach to leverage unlabeled data. Semixup relies on consistency regularization using in- and out-of-manifold samples, together with interpolated consistency. On an independent test set, our method significantly outperformed other state-of-the-art SSL methods in most cases. Finally, when compared to a well-tuned fully supervised baseline that yielded a balanced accuracy (BA) of $70.9\pm0.8%$ on the test set, Semixup had comparable performance -- BA of $71\pm0.8%$ $(p=0.368)$ while requiring $6$ times less labeled data. These results show that our proposed SSL method allows building fully automatic OA severity assessment tools with datasets that are available outside research settings.

==> responses.tex <==
\onecolumn
\overview{Response Letter to Reviewers}
\newperson{Reviewer 1}{R1}

\question{\\This paper proposed a semi-supervised learning (SSL) approach to leverage unlabeled data algorithm for Knee osteoarthritis severity assessment, which relied on consistency regularization using in- and out-of-manifold samples, together with interpolated consistency. In addition, the authors proposed a novel Separable Adaptive Max-pooling replacement for the Global Average Pooling. From the experimental results, the algorithm proposed by the authors performed well. The work is very meaningful, but lacking some innovations in algorithms. }

\answer{\\We  appreciate the reviewer’s feedback and the provided insightful comments, which we addressed below in a point-to-point manner.} 

\question{\\In the abstract, the author pointed out that the proposed method even achieved a comparable performance to a well-tuned fully supervised learning (SL) model that required over 12 times more labeled data, which is not convincing, and needs more experiments to prove.} 

\answer{\\%We apologize for the ambitious statement. 
We have now
provided
%used better 
results with $1000$ labeled samples per KL grade. The comment was addressed by modifying the abstract starting line \ref{ln:data_efficient_edit}, and also adding the text starting line \ref{ln:data_efficient_1} in Discussion (\cref{sc:dis_conc}).} 

\question{\\The loss function in this paper includes cross entropy loss and combination loss without the involvement of labels, and the combination loss includes multiple consistency losses, each of which plays a positive role in the experiment. But it is not clear how to balance these terms in practice, and the experiments should do a better job of evaluating all of these options thoroughly.}

\answer{\\We thank the reviewer for this comment. We agree that more details on the relative importance of each term in the loss function would improve the paper. Therefore, we have conducted an ablation study, in which we have shown how the weighting coefficients in the loss affect the performance of our method on the validation set (\cref{fig:weight_grid_search} and \cref{fig:weight_grid_search_iom}). A detailed description of this experiment is presented in \cref{sc:reg_coef_semixup}.}


\question{\\In data pre-processing, the author used BoneFinder localize the anatomical landmarks and crop the ROIs of $140mm \times 140mm$ centered at each knee joint. Does the precise location of ROI play a role in the experiment? }

\answer{\\Thanks for the question about the pre-processing step. We used BoneFinder to fix possible factors not related to our method, and to be in line with previous work. Ultimately, we think that a sensitivity analysis could be done; however, we point to the study by Tiulpin~\etal~(2018)~[21], which relied on another method that localizes knees accurately to a certain degree, but it still yielded the good performance. 
% In the same study, however, Tiulpin~\etal~pointed out that some of the images’ ROIs had to be removed / corrected due to the failure of the localization method. Therefore, we conclude that accurate ROI localization is not required, but a robust classification rather is. 
% In addition, as we had a possibility of using BoneFinder (a very robust tool according to our experience), the accuracy of localization came rather as a secondary outcome. 
In addition, we have mentioned the robustness of BoneFinder starting line \ref{ln:bonefinder},
Moreover, we want to highlight that similarly to Tiulpin~\etal, we used jittering (random cropping augmentation) in our pipeline, which made our trained model not sensitive to possible inaccuracies of localization.}

\question{\\In addition to this, after intensity standardization, the authors cropped the image again. What's the purpose of this? Will it reduce the effect of standardization if image intensity is standardized and then crop?}

\answer{\\Thanks for this comment. Our motivation of this step was to compare to the method proposed by Tiulpin~\etal~[21] and the answer is similar to above. We have clarified that in lines \ref{ln:preprocessing_in_line_21} and \ref{ln:second_crop}. While we acknowledge that the reviewer is right and the pre-processing step could have been simplified, we believe that it is beyond the scope of our work, as its main focus is Semi-Supervised Learning. We have mentioned in the text starting line \ref{ln:preprocessing_order}.}

\question{\\In Table 2 of the experimental part, the authors experimented with three different pooling methods including GAP, SAM-VH and SAM-HV respectively. It can be seen from the experimental results that the three different pooling methods have the optimal results according to the different number of samples. At the same time, from the average results, GAP method is close to or even better than one of SAM methods. Such results do not seem to prove the advantages of SAM. }

\answer{\\We thank the reviewer for the opportunity to reinforce the clarity of the paper. However, we point out that \cref{tbl:ablation_pooling} corresponds to the model selection, and the results have been computed using labeled data only. We also highlight that we made the final conclusion by looking at the average performance across multiple data settings. To clarify this further, we modified line~\ref{ln:sam_edit1}. 

We would also like to clarify our reasoning on SAM's effectiveness. To assess the validity of the model selection, we still included top-3 fully supervised models selected from our model vs the one by Tiulpin~\etal~trained with different poolings. We showed the performance of these models on the test set in \cref{tbl:sl_ssl_summary} for sanity check, which confirmed our beliefs about the effectiveness of the proposed pooling scheme.}

\question{\\In addition, SAM-VH and SAM-HV differ greatly in different basic methods. In essence, what is the difference between SAM-HV and SAM-VH?}

\answer{\\This comment is partly answered in our previous reply. The conceptual difference between SAM-HV and SAM-VH is such that in the former case, we first pool the features horizontally, and the latter -- vertically. We have previously highlighted this difference in~\cref{fig:sam_all} and also in~\cref{sc:sam} (see lines \ref{ln:sam_clarification}).}

\newpage
\newperson{Reviewer 2}{R2}

\question{\\The authors present novel semi-supervised learning called semixup with applications on KL grading of OA. The paper is very well written. }

\answer{\\We are thankful for your feedback.}

\question{\\
In the paper Fig.3 is called Fig.2}

\answer{\\We carefully searched and rechecked the paper several times, and ensured that the figure indices are correct. }

\question{\\In section B of the methods, the authors mention "Each branch of this model generates $1\times1$ features, which are concatenated". \\Is that correct? Shouldn't it be $16\times16$?}

\answer{\\We indeed mean it because the input of SAM is a $16\times16$ feature map, and it is first pooled into a vector with the shape of either $1\times 16$ or $16\times 1$. This is subsequently passed through a non-linearity and finally pooled into a $1\times1$ feature map. Besides the line \ref{ln:sam} and \Cref{tbl:detailed_arch}, we have clarified it in the texts starting lines \ref{ln:sam_output} and \ref{ln:sam_edit}.}

\question{\\Fig.7 It would help the readers if the ROC values are added in the caption.}

\answer{\\Thanks for the valuable suggestion. We agree. As it is important to present confidence intervals for the AUC and AP values, the caption becomes overloaded. Hence, we moved them into \cref{tbl:comparison_many_metrics}, which is right above the corresponding section and \cref{fig:semixup_roc_auc}.}

\newpage
\newperson{Reviewer 3}{R3}

\question{\\
The paper is very well structured and written, good to understand and the technical presentation is sound. Both aspects of the paper (methodological and applicational) come with sufficient novelty and perfectly fit the scope of TMI. The used large-scale datasets (OAI and MOST) are publicly available as well as the proposed models (published on github). I consider this an important factor to allow for independent comparison and a higher impact.}

\answer{\\
We are thankful for your feedback and insightful comments.}

\question{\\
The manuscript is already pretty mature and I don't see any principle obstacles that would prohibit a publication; however, I have some comments the authors should address before publication:
II A: 'The second limitation of the aforementioned studies is that only the number of labeled samples was varied in the experiments; however, none of them explored the amount of unlabeled data needed to achieve good performance. We emphasize the importance of this issue in medical imaging as from one application to another, the amounts of both labeled and unlabeled data can differ.'
This statement above leaves me a little unsatisfied when I have a look at Table S8 in the supplement. The table shows all classification results for all compared SSL setups on the MOST test set in a 5-fold cross-validation study with each fold consisting of 24 data settings varying the amount of labeled an unlabeled data used for training. I can't figure out a general trend on how many unlabeled data is suitable, especially the results for the proposed Semixup method varies a lot and in a not-simple-to-grasp fashion with varying amount of unlabeled data (see e.g. col 1000). Do the authors have ideas how to explain this behavior? How is the data organized, are the different settings cascaded subsets or are they disjoint? From my perspective cascaded subsets are a more natural choice since they add some more data from setting to setting and should not. What makes me even wonder more is the Semixup result in row-block 5N, since the performance decreases from 65.9 (col 500) to 61.7 (col 1000). More labeled data for training leads to a less performing model? This is strange.}

\answer{\\We thank the reviewer for the opportunity to provide stronger evidence to support the statement 'The second limitation of … data can differ'. We thank the reviewer for this comment, and we think that addressing it has significantly improved our manuscript. Our first changes regarding this statement can be seen in Introduction starting line~\ref{ln:intro_limitation}.

After running 9 extra experiments with different random seeds, we now report more robust and evident trend of performance scaling in \Cref{suptab:results-all}. Specifically, we now show that having $1N$ unlabeled is sufficient and the performance of all the SSL methods did not change substantially with the increase of the amounts of unlabeled data in our experiments. This point is further stressed in Discussion starting line~\ref{ln:discussion_methodological_impact}. Additionally, we point out that~\Cref{suptab:results-all} shows the results on the test set, and not the model selection ones as anticipated by the reviewer.

Thanks for the 
%We respect the 
comment about the cascaded splitting. %This is one way to conduct the experiments. Another way is 
We have chosen to treat the balanced accuracy on the test set as a random variable, and conduct multiple independent runs with different random seeds (each time with a different data split). We have graphically illustrated the process of data splitting in \Cref{fig:oai_splitting_workflow} and \Cref{suptab:results-all} has now the results evaluated in this manner. 

With regard to the last comment, as now the results in \Cref{suptab:results-all} are more robust,  the performance drop previously seen the increase of labeled data is not anymore observed. %Therefore, we conclude that the previous confusion was merely caused by computational instability of calculations, and we once again apologize for this, and thank the reviewer for this comment.
}
% \answer{
% Firstly, we are sorry and fully agree that we didn’t provide empirical evidence to support that point 'The second limitation of … data can differ’. So, we revised it in red.
% Regard to the matter of \Cref{suptab:results-all}, we actually evaluated a single model per method after training each method once. That would explain the instability of the results. Thanks to the reviewer’s concern, we rerun all the settings there 9 more times. In each new experiment, we randomly sampled a seed that affects data sampling and weight initialization. We refined \Cref{suptab:results-all} by reporting averages and standard errors of the 10 iterations. The table now shows much more stable results. Importantly, we empirically prove our method’s strength when it surpasses other state-of-the-art SSL methods in most of the cases.
% With respect to the way we organized data, we treated the data settings independently. We provided a graphical illustration of data splitting in \Cref{fig:oai_splitting_workflow}.}

\question{\\
This is also a point where some general criticism applies. Especially for the knee OA scoring, as we can see with your SL results, there is enough labeled data available to perform simple supervised learning. Indeed, your results imply that there is (in the sense of there exists) a SSL configuration that performs as good as the SL configuration (71 vs 70.9 mean balanced accuracy), but this configuration of cause is not guaranteed to be found easily without extensive testing. That means if one wants to simply set up a classification pipeline without any interest in technical details (and sugar) your results suggest that the supervised approach is preferable since for the sake of simplicity.}

\answer{\\We thank the reviewer for this question. One may argue that a similar criticism applies for all state-of-the-art general-purpose SSL methods since all of them have hyperparameters that need to be tuned for every application.  We now discuss this point in Discussion starting line \ref{ln:dis_ssl_limitation}. We note however that the comparison in \cref{tbl:sl_ssl_summary} is between a SL method trained on 31,922 images while the SSL approach had only 1000 labels / KL grade showing that Semixup provides a large statistical advantage in the number of required labels. 

% What our paper really aims to answer are the following questions:
% \begin{itemize}
%     \item How many radiographs one should annotate to make a clinically applicable OA grading model?
%     \item Should we use all available unlabeled data?
% \end{itemize}

}

\question{\\
IV B: You used BoneFinder to detect the ROI the knee. I wonder how many failed detections you have and how you handled them. Since I know the very much varying x-ray quality of the PA bilateral images from the OAI database (e.g. missing half legs), I would like to know more details on how you excluded OAI data. Did you also exclude OAI images with implants? You stated it for the MOST data but I can't find a similar note on the OAI data.}

\answer{\\
We did not find any failed detections since BoneFinder seems to be a robust tool. We have clarified its performance in the sentences starting line \ref{ln:bonefinder}. See also our response to R1.4.

Our inclusion criteria comprised the exclusion of implants (i.e., total knee replacement at baseline), and also the cases which did not have the present KL grades. We have clarified this in the text starting line \ref{ln:oai_data_filter}, and revised the first paragraph of \cref{sc:datasets}. Moreover, we have modified \Cref{fig:oai_splitting_workflow} to support both the answers above.
% However, we have also taken some additional measures to prevent the failure of detection such as prior the localization, we applied zero padding (300 pixels on image side of every image). We note that 2 images could not be read by pydicom, which we used for DICOM image processing, and we excluded them. We have added a footnote related to it in the text starting line \ref{ln:data_exclusion_footnote}.  
%Since these are rather technical details, and has limited relevance to the core of our work (new semi-supervised learning method), we decided to not overload the reader with those details.
}
% \answer{\\
% Firstly, the step credits to Tiulpin et al. [21]. We manually verified that all cropped images containing whole left/right knees translated by a certain range. In other words, we’d safely say that the left-most and right-most edges of the tibia and the femur of each knee are preserved during the cropping.
% As mentioned in the Datasets section, we used the OAI’s baseline, and its follow-up visits after 12, 18, 24, 30, 36, 48, 60, 72, 84, 96, 108, 120, and 132 months. In addition, we removed knees that were annotated with KL out of the range [0, 4], which excludes images with invalid annotation or TKR.}

\question{\\
IV B: The whole data processing pipeline is very application specific to PA knee x-rays. Please discuss some appropriate actions that could generalize your method and especially again explicitely point on the application invariant core ideas.}

\answer{\\
As the scope of our study was PA knee radiographs, we concentrated on such data only. We discussed more about utilizing Semixup to other applications in the text starting line \ref{ln:apply_semixup_to_others} in \cref{sc:dis_conc}.}

\question{
IV B 2: I miss some more details on the data split. Was it done randomly? If not, what were the rules applied to generate it?}

\answer{\\
We thank the reviewer for this comment and apologize for the lack of clarity. We have graphically illustrated the data splitting process in \Cref{fig:oai_splitting_workflow}, and also better highlighted it in the text in line \ref{ln:data_split_edit}.}

\question{\\Table II: The caption lacks some explanation of the bold and underlined entries. \\
Table IV: In column 100 the first three row show the same values. I guess this is a copy and paste error. Please check carefully. \\
V. 'We highlight that this work demonstrates results drastically outperforming all the previous studies on automatic KL grading'. Well, your results are pretty good and I know that one has to sell the own work sufficiently but please rephrase this statement and make it sound a little bit more moderate. \\
Table S8 caption: ...(BA, $\%$) ON AN INDEPENDENT TEST SET  DATA FOR ALL THE SL AND SSL MODELS.' I only see results for the SSL setups, am I missing something here?}

\answer{\\
We thank the reviewer for pointing out the typos. 
\begin{enumerate}
    \item We have fixed the caption of \cref{tbl:ablation_pooling} and explain the bold and the underlined entries.
    \item Table IV (now \cref{tbl:ablation_loss}) has correct results. The confusion may have occurred due to rounding.
    \item We have moderated the enthusiasm of our presentation. %We absolutely agree with the reviewer about the "superiority" statement. Thus, we have removed it in the revised manuscript.
    \item Finally, we note that the caption of \Cref{suptab:results-all} has been corrected.
\end{enumerate}
}

\question{\\
One last point:
What happens if you consider even more labeled cases? It seems as if saturation (compared to the supervised full OAI model) is reached, but as I'm a curious person I ask myself whether you have tried a larger portion of labeled cases and if so, what was the outcome? In general a discussion on the 'right' amount of labeled data in an SSL setup is desirable, because since labeling is expensive one does not want to label more data than necessary to reach a certain saturation. The size of OAI and MOST database offers you this unique opportunity for such an investigation.}

\answer{\\
We thank the reviewer for this valuable comment and we have added \Cref{sc:more_labeled_data} highlighting the saturation of performance when increasing the amount of labeled data. We now mentioned these new results starting line~\ref{ln:more_data_note} in the manuscript.}

==> revision_summary.tex <==
\onecolumn
\overview{[TMI-2020-0340] Revision Summary}

\begin{table}[htbp]
\renewcommand\thetable{}
\centering
\renewcommand{\arraystretch}{1.5}
\caption{}
\begin{tabular}{|r|l|l|l|l|}
\hline
\multicolumn{1}{|l|}{\textbf{ID}} & \textbf{Section} & \textbf{Line/Reference} & \textbf{Changes} & \textbf{Related comments} \\ \hline
1 & \multicolumn{ 1}{l|}{Abstract} & \ref{ln:abs_wording_1} & Wording &  \\ \cline{ 1- 1}\cline{ 3- 5}
2 & \multicolumn{ 1}{l|}{} & \ref{ln:data_efficient_edit} & Replaced the result & R1.2 \\ \hline
3 & \multicolumn{ 1}{l|}{Introduction} & \ref{ln:intro_wording_1}, \ref{ln:intro_wording_2} & Wording &  \\ \cline{ 1- 1}\cline{ 3- 5}
% 4 & \multicolumn{ 1}{l|}{} &  &  &  \\ \cline{ 1- 1}\cline{ 3- 5}
4 & \multicolumn{ 1}{l|}{} & \cref{fig:samples_by_kl} & Corrected the caption &  \\ \hline
5 & \multicolumn{ 1}{l|}{Related work} & \ref{ln:intro_limitation} & Modified the statement & R3.2 \\ \cline{ 1- 1}\cline{ 3- 5}
6 & \multicolumn{ 1}{l|}{} & \ref{ln:rw_wording_1} & Wording &  \\ \hline
7 & \multicolumn{1}{l|}{Method} & \ref{ln:sam_output}, \ref{ln:sam_edit} in \cref{sc:sam} & Clarified the output shape of SAM & R2.3 \\ \hline
8 & \multicolumn{ 1}{l|}{Experiments} & First paragraph in \cref{sc:datasets} & Clarified the process of data preparation  & R3.4 \\ \cline{ 1- 1}\cline{ 3- 5}
9 & \multicolumn{ 1}{l|}{} & \ref{ln:exp_typo_1} & Fixed the typo &  \\ \cline{ 1- 1}\cline{ 3- 5}
10 & \multicolumn{ 1}{l|}{} & \ref{ln:bonefinder} & Clarified the robustness of BoneFinder & R1.4, R3.4 \\ \cline{ 1- 1}\cline{ 3- 5}
11 & \multicolumn{ 1}{l|}{} & \ref{ln:preprocessing_in_line_21}, \ref{ln:second_crop} & Clarified that our pre-processing step was in line with [21] & R1.5 \\ \cline{ 1- 1}\cline{ 3- 5}
12 & \multicolumn{ 1}{l|}{} & \ref{ln:data_split_edit} & Referenced to \Cref{fig:oai_splitting_workflow} & R3.4, R3.6 \\ \cline{ 1- 1}\cline{ 3- 5}
13 & \multicolumn{ 1}{l|}{} & \ref{ln:sam_edit1} & Clarified the architecture selection related to SAM & R1.6 \\ \cline{ 1- 1}\cline{ 3- 5}
14 & \multicolumn{ 1}{l|}{} & \ref{ln:remove_not_relavence} & Removed the irrelevant paragraph after updating \Cref{suptab:results-all} &  \\ \cline{ 1- 1}\cline{ 3- 5}
15 & \multicolumn{ 1}{l|}{} & \cref{sc:compare_sl_ssl} & Restructured the subsection by moving Section D-2 out of it &  \\ \cline{ 1- 1}\cline{ 3- 5}
16 & \multicolumn{ 1}{l|}{} & \ref{ln:ssl_0x_update1}, \ref{ln:ssl_0x_update2} & Improved the readability &  \\ \cline{ 1- 1}\cline{ 3- 5}
17 & \multicolumn{ 1}{l|}{} & \ref{ln:sl_ssl_typo1} & Typo &  \\ \cline{ 1- 1}\cline{ 3- 5}
18 & \multicolumn{ 1}{l|}{} & \ref{ln:more_data_note} & Clarified results with more labeled data & R3.8 \\ \cline{ 1- 1}\cline{ 3- 5}
19 & \multicolumn{ 1}{l|}{} & \cref{sc:ablation_study} & Added the new section & R1.3 \\ \cline{ 1- 1}\cline{ 3- 5}
20 & \multicolumn{ 1}{l|}{} & \cref{sc:ablation_clustering} & Moved Section IV-D.2 to \cref{sc:ablation_clustering} & R1.3 \\ \cline{ 1- 1}\cline{ 3- 5}
21 & \multicolumn{ 1}{l|}{} & \cref{sc:reg_coef_semixup} & Added the new section & R1.3 \\ \cline{ 1- 1}\cline{ 3- 5}
22 & \multicolumn{ 1}{l|}{} & \cref{tbl:ablation_pooling} & Corrected the caption & R3.7 \\ \cline{ 1- 1}\cline{ 3- 5}
23 & \multicolumn{ 1}{l|}{} & \cref{fig:weight_grid_search}, \cref{fig:weight_grid_search_iom} & Added the new figures about coefficient balancing & R1.3 \\ \hline
24 & \multicolumn{ 1}{l|}{Discussion} & \ref{ln:data_efficient_1} & Updated a conclusion about the label-efficiency of Semixup & R1.2 \\ \cline{ 1- 1}\cline{ 3- 5}
25 & \multicolumn{ 1}{l|}{and Conclusions} & \ref{ln:apply_semixup_to_others} & Added a discussion about applying Semixup & R3.5 \\ \cline{ 1- 1}\cline{ 3- 5}
26 & \multicolumn{ 1}{l|}{} & \ref{ln:dis_wording_1}, \ref{ln:dis_wording_2} & Wording &  \\ \cline{ 1- 1}\cline{ 3- 5}
27 & \multicolumn{ 1}{l|}{} & \ref{ln:dis_remove_1} & Removed a sentence to moderate our enthusiasm  & R3.7 \\ \hline
28 & \multicolumn{ 1}{l|}{Supplement} & & Reset the index count of the figures and tables & \\ \cline{ 1- 1}\cline{ 3- 5}
29 & \multicolumn{ 1}{l|}{} & \ref{ln:sup_typo_1} & Typo &  \\ \cline{ 1- 1}\cline{ 3- 5}
30 & \multicolumn{ 1}{l|}{} & \Cref{suptab:results-all} & Corrected caption and update values after running 9 more iterations & R3.2 \\ \cline{ 1- 1}\cline{ 3- 5}
31 & \multicolumn{ 1}{l|}{} & \Cref{sc:more_labeled_data} & Added the new section “More labeled data” & R3.8 \\ \cline{ 1- 1}\cline{ 3- 5}
32 & \multicolumn{ 1}{l|}{} & \Cref{fig:semixup_by_nlabels} & Added the new figure about “More labeled data” & R3.8 \\ \cline{ 1- 1}\cline{ 3- 5}
33 & \multicolumn{ 1}{l|}{} & \Cref{fig:oai_splitting_workflow} & Updated the figure to clarify OAI data selection and splitting & R3.2, R3.4, R3.6 \\ \hline
\end{tabular}
\end{table}


